CroMo: Cross-Modal Learning for Monocular Depth Estimation

Learning-based depth estimation has witnessed recent progress in multiple directions; from self-supervision using monocular video to supervised methods offering highest accuracy. Complementary to supervision, further boosts to performance and robustness are gained by combining information from multiple signals. In this paper we systematically investigate key trade-offs associated with sensor and modality design choices as well as related model training strategies. Our study leads us to a new method, capable of connecting modality-specific advantages from polarisation, Time-of-Flight and structured-light inputs. We propose a novel pipeline capable of estimating depth from monocular polarisation for which we evaluate various training signals. The inversion of differentiable analytic models thereby connects scene geometry with polarisation and ToF signals and enables self-supervised and cross-modal learning. In the absence of existing multimodal datasets, we examine our approach with a custom-made multi-modal camera rig and collect CroMo; the first dataset to consist of synchronized stereo polarisation, indirect ToF and structured-light depth, captured at video rates. Extensive experiments on challenging video scenes confirm both qualitative and quantitative pipeline advantages where we are able to outperform competitive monocular depth estimation method.

==> 04_related_03.tex <==
%\subsection{Polarisation}

% \noindent The polarisation of light is affected by reflection from object surfaces linking polarisation measurements intrinsically to surface normals. This link can be leveraged to estimate normals or depth. Inferring depth from a single polarisation image, without any additional information, remains challenging due to the ill-posed nature of the problem that results from intrinsic physical ambiguities.

%\noindent\textbf{Learning based Pol. }
%Due to lack of available datasets, only a limited number of works focus on learning with polarisation. leveraging polarisation through learning pipelines. %Probably because of the complicated access to large dataset of polarized images like \cite{shi2016benchmark}. 
%This can be primarily attributed to the compounding effects of data hungry contemporary methods and a distinct lack of large, available polarisation image sets. Ba \etal~\cite{ba2019physics} consider polarisation images and a set of candidate normals, deduced from the physical Fresnel equations. They design a simple supervised network to disambiguate and refine polarisation normals. More recently deep polarisation networks have been developed to address common task failure cases, typically observed in networks that use only RGB imagery. Kalra \etal~\cite{kalra2020deep} proposed a method capable of performing instance segmentation of transparent objects while Blanchon \etal~\cite{blanchon2020p2d} improved depth estimation of specular surfaces with the addition of polarisation cues.


%\subsection{Time-of-Flight (i-ToF)}

%The light gets reflected by objects in the scene, and based on the round-trip time, depth from the camera is computed. The intrinsic sensing for the time delay is realized by correlating a series of phase-shifted emitter signals with the reflected light measurements. This produces four \textbf{correlation images} $C_0$, $C_1$, $C_2$, $C_3$ from which the depth is usually estimated leveraging physical models~\cite{noraky2019low} or learning based approaches~\cite{su:2018}. Due to limited size and energy requirements, i-ToF depth maps are typically low resolution, noisy, and contain missing regions (holes).

% i-ToF also suffers from multi-path interference and strong ambient light; however it works well in low-light scenes where passive high-resolution acquisitions struggle.


%when a wave that travels on the direct shortest path interferes with received light that is reflected multiple times within the scene before being detected. 

%i-ToF sensors are available at affordable cost and are an increasingly popular choice for mobile devices, offering portable active depth measurement with high precision for short range distances~\cite{hansard2012time}. However well understood weaknesses include limited spatial resolution, an inability to receive signal from specular surfaces %, due to specular reflections 
%and susceptibility to measurement error~\cite{foix2011lock}. Error comes from multiple sources; zero mean noise (thermal, photon shot) and scene dependent multi-path interference (MPI). The latter arises due to the nature of the sensing strategy; a signal traveling from the source to detector via two (or more) paths results in multiple received components that then interfere (constructively or destructively), manifesting in depth measurement overestimation, % that are farther than reality, 
%noise and artifacts.

%\noindent\textbf{i-ToF depth improvement. }
%MPI can be considered a critical issue and error mitigation has been the focus of a body of work~\cite{whyte2014review}. Early work proposed simplifying assumptions such as two-path approximations that allow for closed-form solutions~\cite{godbaz2012closed} or iterative approaches~\cite{dorrington2011separating,kirmani2013spumic}. Generalisations to multiple bounces have also been considered; Freedman \etal.~\cite{freedman2014sra} proposed an iterative solution by considering multiple frequency measurements and approximate scatter complexity with sparse reflections %assume that reflections are sparse, providing only a weak approximation for scattering complexity, 
%yet experimental work was limited to toy scenes. Kadambi \etal.~\cite{kadambi2013coded} introduce a ‘coded’ illumination technique by re-purposing i-ToF sensors via hardware modification and report MPI correction on scenes with translucent objects. A number of works have also incorporated light transport information to correct for MPI~\cite{o2014temporal,gupta2015phasor,naik2015light,achar2017epipolar}.

%\noindent\textbf{Learning with i-ToF. }
%In common with the polarisation literature; learning approaches are mainly hampered by the lack of available real world data with reliable ground truth depth even though  for improving i-ToF depth estimation have received less attention, due mainly to limited available real world training data and registered depth ground truth. However it has been hypothesized that the majority of MPI information is accessible in image space~\cite{marco2017deepi-ToF} motivating the use of contemporary tools, namely Convolutional Neural Networks (CNN), to explore the efficacy of data-driven error correction and thus alleviate explicit-model requirements, specification of complicated reflection interactions. 
%Son \etal.~\cite{son2016learning} used a robotic arm to collect $540$ real training images of short range scenes (objects on a table), with a structured light sensor providing ground truth labels to their neural network. To mitigate the expense of collecting i-ToF depth and registered ground truth, Marco \etal.~\cite{marco2017deepi-ToF} train an encoder-decoder network %in an unsupervised fashion on real depth maps 
%such that the encoder learns a suitable basis to represent real MPI-corrupted depth images while the decoder obtains supervision to correct depth from synthetically rendered scenes with ground-truth. Synthetic training has also been used to learn raw i-ToF to scene depth mappings in an end-to-end fashion~\cite{su2018deep,guo2018tackling,agresti2018deep} however investigation of the ability to account for real world domain shifts is either missing or limited. In recent work Agresti \etal.~\cite{Agresti_2019_CVPR} employ %synthetic imagery in combination with unlabelled real data, employing 
%a GAN to address %the %noted domain adaption %issue yet acquire only small real data and %with ground-truth and therefore use it only for testing purposes. 


==> _planning.tex <==


%% TO DO CVPR 22 %%

% 1) Remove supervision (L1), minimize RS in text

% 2) Depth Hint vs. fully supervised: Remove supervision from main paper. Put in supplementary material

% 3) Improve visualizations. Maybe include error maps (instead of GT). To overcome GT quality questions.

% 4) Squeeze in fig. from supplementary + rest of rebuttal. Rewrite sharpening part.

% 5) Remove ResNet18 from ablation (maybe?)


Two main claims, mainly supported by Tabs.~\ref{tab:contrib_dataset}, \ref{tab:contrib_architecture}.

\begin{itemize}
% modality interaction?
% explore the sensor-combination-space?
\item \textbf{Claim 1:}

\item We investigate and analyze the value of considering multiple image modalities at training time, for the task of depth estimation. A necessary requirement for exploring this topic involves the collection of our synchronised, video rate multi-modal data. Release of this novel dataset provides an auxiliary contribution; of large benefit to the community for future work on related topics e.g. multi-modal fusion.

%\item We present a \textbf{unique dataset}, that provides rich multi-modal information, originating from multiple, synchronized, video-rate sensors.

%\ben{I'd probably go like: "We investigate the use of multiple image modalities for the task of depth estimation." And see the dataset rather as the vessel to do so. The necessity of having it synced and with video rate data is then just a necessary requirement to investigate these things. That would make the investigation / study / analysis of multiple modalities the claim and the dataset an auxiliary contribution for doing this that can benefit future research on e.g. multi-modal fusion.}

\begin{itemize}

\item Tab.~\ref{tab:contrib_dataset} explores the improvements afforded to monocular depth estimation when increasing the number of sensors available at training time.

\item Take-away message: more sensors, more training information, better depth. 

\item Our exploration of potential improvements, from configuration changes in sensor-space, is valuable and uniquely made possible by our dataset contribution. 
\item \ben{Every sensor has its own disadvantages / benefits. Understand where a specific modality helps / where its use is problematic etc. We can support this with qualitative back up.} \sgm{Can we find these qualitative examples? (hard)}

\end{itemize}

\item \textbf{Claim 2:}

\item Our \textbf{novel Method} provides sharper and more accurate depth estimation.

\begin{itemize}

\item Our Model is composed of a novel architecture with a dedicated sharpener module and two novel analytical loss terms.

\item Tab.~\ref{tab:contrib_architecture} shows the benefit of our method \emph{c.f.} larger competing models; Midas.

\item Take-away message: each component of our model is beneficial to performance, especially the flow.

\item By fixing a consistent architecture, the \textbf{ablation study} highlights that our novel analytical loss improves depth estimation quality.

\end{itemize}

\end{itemize}

\noindent We select to \underline{not discuss} \emph{full supervision} and \emph{self-supervision} distinctions, since using i-ToF can be considered as supervised learning, or as using ''depth hints''. 


We select to strictly \underline{not discuss} RGB imagery. This opens the door to comments, suggestions on exploring depth estimation performance with other common RGB datasets, which we aim to avoid. One unique aspect of our CroMo dataset is it constitutes the first pubic dataset with stereo polarisation.

We specifically only discuss our findings, uniquely made possible by considering our dataset. That is, more sensors, with various modalities, are able to meaningfully improve the depth prediction.
\newline
\newline
\noindent \textbf{TO DO (non-text)}
\small
\begin{itemize}
\item Update Fig1 (Teaser)            % $\checkmark$
\item Image-Table Figure              % $\checkmark$
\item Arch+Loss Figure                % $\checkmark$
\item Kitti RGB expr (Supp.)          % $\checkmark$
\item Video generation script (Supp.) % $\checkmark$
\end{itemize}

\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{gfx/intro/20201027_181125_0000000209.png}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{gfx/intro/20201027_181125_0000000567.png}
\end{figure}
